Sketching, Embedding, and Dimensionality Reduction for Information Spaces

Information distances like the Hellinger distance and the Jensen-Shannon divergence have deep roots in information theory and machine learning. They are used extensively in data analysis especially when the objects being compared are high dimensional empirical probability distributions built from data. However, we lack common tools needed to actually use information distances in applications efficiently and at scale with any kind of provable guarantees. We can't sketch these distances easily, or embed them in better behaved spaces, or even reduce the dimensionality of the space while maintaining the probability structure of the data. In this paper, we build these tools for information distances---both for the Hellinger distance and Jensen--Shannon divergence, as well as related measures, like the $\chi^2$ divergence. We first show that they can be sketched efficiently (i.e. up to multiplicative error in sublinear space) in the aggregate streaming model. This result is exponentially stronger than known upper bounds for sketching these distances in the strict turnstile streaming model. Second, we show a finite dimensionality embedding result for the Jensen-Shannon and $\chi^2$ divergences that preserves pair wise distances. Finally we prove a dimensionality reduction result for the Hellinger, Jensen--Shannon, and $\chi^2$ divergences that preserves the information geometry of the distributions (specifically, by retaining the simplex structure of the space). While our second result above already implies that these divergences can be explicitly embedded in Euclidean space, retaining the simplex structure is important because it allows us to continue doing inference in the reduced space. In essence, we preserve not just the distance structure but the underlying geometry of the space.

==> proofs.tex <==
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "170"
%%% End:

